On Free Description Logics with Definite Descriptions

Definite descriptions are phrases of the form 'the $x$ such that $\varphi$', used to refer to single entities in a context. They are often more meaningful to users than individual names alone, in particular when modelling or querying data over ontologies. We investigate free description logics with both individual names and definite descriptions as terms of the language, while also accounting for their possible lack of denotation. We focus on the extensions of $\mathcal{ALC}$ and, respectively, $\mathcal{EL}$ with nominals, the universal role, and definite descriptions. We show that standard reasoning in these extensions is not harder than in the original languages, and we characterise the expressive power of concepts relative to first-order formulas using a suitable notion of bisimulation. Moreover, we lay the foundations for automated support for definite descriptions generation by studying the complexity of deciding the existence of definite descriptions for an individual under an ontology. Finally, we provide a polynomial-time reduction of reasoning in other free description logic languages based on dual-domain semantics to the case of partial interpretations.

==> 10.2-sec_app_prelim.tex <==
\subsection*{Proofs for Section~\ref{sec:freedl}}


We show that
$\Lmc$
%$\ALCOud$
ontology satisfiability on partial interpretations is reducible to
%$\ALCOud$
$\Lmc$
ontology satisfiability on total interpretations, where $\Lmc \in \{ \ALCOud, \ELOud \}$.
%Together
%Since the proof for $\ELOud$ is analogous,
Together with the observation
%showing
that the viceversa holds as well, this implies
%the desired result of
Theorem~\ref{thm:interred}.

%To see this,
Given an
$\Lmc$
%$\ALCOud$
concept $C$
%(with $\top$ now defined by $\lnot \bot$)
and an ontology $\Omc$,
%
let $\De$ be a fresh concept name, standing for the
\emph{denotation concept},
that does not occur in $C$ and $\Omc$.
%
We define the translation $\cdot^{\derel}$,
%called \emph{existence relativisation},
mapping an
%$\ALCOud$
$\Lmc$
concept $C$ to an
$\Lmc$
%$\ALCOud$
concept $C^{\derel}$ as follows, where $s \in \NR \cup \{ u \}$:
%We introduce the translations $\cdot^{+}$, respectively $\cdot^{-}$, that map an $\ALCO$ concept $C$ to an $\ALCO$ concept $C^{+}$, respectively $C^{-}$, as follows:
%
%\begin{gather*}
%	A^{\derel} = A, \quad
%	\{ \tau \}^{\derel} = \{ \tau \}, \quad
%%	\top^{\derel} = \De, \quad
%	(\lnot C)^{\derel} = \lnot C^{\derel}, \\
%	(\exists r. C)^{\derel} = \exists r.(\De \sqcap C^{\derel}), \quad
%	(C \sqcap D)^{\derel} = C^{\derel} \sqcap D^{\derel}.
%\end{gather*}
\begin{gather*}
	\bot^{\derel} = \bot, \ \top^{\derel} = \De \sqcap \top, \
	A^{\derel} = \De \sqcap A, \\
%	\{ \tau \}^{\derel} = \De \sqcap \{ \tau^{\derel} \}, \quad
%	\{ \tau \}^{\derel} = \{ \tau^{\derel} \}, \quad
	\{ a \}^{\derel} = \De \sqcap \{ a \}, \
	\{ \defdes D \}^{\derel} = \{ \defdes(\De \sqcap D^{\derel}) \}, \\
%	\top^{\derel} = \De, \quad
	(\lnot C)^{\derel} = \lnot C^{\derel}, \
	(C \sqcap D)^{\derel} = (C^{\derel} \sqcap D^{\derel}), \\
%	(\lnot C)^{\derel} = \De \sqcap \lnot C^{\derel}, \\
%	(\exists r. C)^{\derel} = \exists r.(\De \sqcap C^{\derel}), \quad
	(\exists s. C)^{\derel} = \De \sqcap \exists s.(\De \sqcap C^{\derel}).
%	(C \sqcap D)^{\derel} = \De \sqcap (C^{\derel} \sqcap D^{\derel}),
\end{gather*}
%where, for an individual name $a$, we set $a^{\derel} = a$, while, for a definite description $\defdes D$, we define $(\defdes D)^{\derel} = \defdes (\De \sqcap D^{\derel})$.
%
%Finally, we consider the translation $\cdot^{\star}$ defined as above, but now mapping $\ALCOd$ formulas to $\ALCOd$ formulas.
%For $\ELOud$, we set also $\bot^{\derel} = \bot$ and $\top^{\derel} = \De \sqcap \top$.
Moreover, we extend the function $\cdot^{\derel}$
%so to map an
to $\ALCOud$ CIs
%\footnote{Recall that, without loss of generality (cf. Section~\ref{sec:observations}), we can assume that an $\ALCOd$ formula does not take the form of an $\ALCOd$ assertion.}
%$\Omc$
%to an $\ALCOud$ CI
%$\Omc^{\derel}$
as
\begin{gather*}
(C \sqsubseteq D)^{\derel} = \De \sqcap C^{\derel} \sqsubseteq D^{\derel},
%\\
%		(\lnot \p)^{\derel} = \lnot \p^{\derel}, \
%		(\p \land \psi)^{\derel} = \p^{\derel} \land \psi^{\derel}
\end{gather*}
and finally we set (assuming without loss of generality, cf. First Remarks, that $\Omc$ does not contain assertions):
\[
\Omc^{\derel} = \bigcup_{C \sqsubseteq D \in \Omc} \{ (C \sqsubseteq D)^{\derel} \} \cup \{ \top \sqsubseteq \exists u.\De \}.
\]
%
We then have the following result.


\begin{restatable}{lemma}{partintdualdom}
\label{prop:partintdualdom}
%\nb{M: changed, to check}
Let $\Omc$ be an
$\Lmc$
%$\ALCOud$
ontology, with $\Lmc \in \{ \ALCOud, \ELOud \}$.
There exists a partial interpretation $\Imc$ such that $\Imc \models \Omc$ iff there exists a total interpretation $\Jmc$ such that $\Jmc \models \Omc^{\derel}$.
\end{restatable}
%
%
\begin{proof}
\nb{M: changed, to check}
%\nb{M: move to `Proofs for Sec. 2'?}
To prove the statement, we assume without loss of generality that $\Omc$ does not contain assertions (cf. Section~\ref{sec:observations}) and show the following.
\begin{enumerate}
[label=$(\roman*)$, align=left, leftmargin=*, labelsep=0cm]

\item For every partial interpretation $\Imc$ such that $\Imc \models \Omc$, there is a total interpretation $\Imc^{'}$ 
%	coinciding with $\Imc$ on the interpretation of all concept and role names in $\p$, as well as on the interpretation of all individual names in $\p$ that denote in $\Imc$, and
	such that
$
	\Imc^{'} \models \Omc^{\derel}.
$

	\item For every total interpretation $\Jmc$ such that
$
\Jmc \models \Omc^{\derel},
$
	there is a partial interpretation $\Jmc'$
%	coinciding with $\Jmc$ on the interpretation of all concept, role and individual names in $\p$ and
	such that
	$\Jmc' \models \Omc$.
\end{enumerate}

$(i)$
Let $\Imc = (\Delta^{\Imc}, \cdot^{\Imc})$ be a partial interpretation such that $\Imc \models \Omc$.
We construct a total interpretation $\Imc' = (\Delta^{\Imc'}, \cdot^{\Imc'})$ such that:
$\Delta^{\Imc'} = \Delta^{\Imc} \cup \{ d_{u} \}$ (where $d_{u} \not \in \Delta^{\Imc}$);
$\De^{\Imc'} = \Delta^{\Imc}$;
for every $A \in \NC \setminus \{ \De \}$, $A^{\Imc'} = A^{\Imc}$;
for every $r \in \NR$, $r^{\Imc'} = r^{\Imc}$;
and for every $a \in \NC$,
$a^{\Imc'} = a^{\Imc}$, if $a$ denotes in $\Imc$, while $a^{\Imc'} = d_{u}$, otherwise.
Clearly, $\Imc' \models \top \sqsubseteq \exists u.\De$.
We now claim the following.
%
\begin{claim}
  For all $C \in \con{\Omc}$ and $d \in \Delta^{\Imc'}$, $d \in C^{\Imc}$
  iff $d \in (C^{\derel})^{\Imc'}$.
%  For all $C \in \con{\p}$ and $d \in \Delta^{\Imc}$, $d \in C^{\Imc}$
%  iff $d \in (C^{\derel})^{\Imc'}$.
\end{claim}
%
\begin{proof}
The proof is by induction on $C$. The base cases are as follows.
%
\begin{itemize}
\item For $C = \bot$, $d \in \bot^{\Imc}$ iff $d \in \bot^{\Imc'}$, i.e., $d \in (\bot^{\derel})^{\Imc'}$.
\item For $C = \top$, we have $d \in \top^{\Imc}$ iff $d \in \Delta^{\Imc} \cap \top^{\Imc}$, i.e., $d \in (\De \sqcap \top)^{\Imc'}$, by
  definition of $\Imc'$. By definition of $\cdot^{\derel}$, this means that $d \in (\top^{\derel})^{\Imc'}$.
\item For $C = A$, we have $d \in A^{\Imc}$ iff $d \in \Delta^{\Imc} \cap A^{\Imc}$, which is equivalent to $d \in (\De \sqcap A)^{\Imc'}$, by
  definition of $\Imc'$. By definition of $\cdot^{\derel}$, the previous step means that $d \in (A^{\derel})^{\Imc'}$.
%
\item For $C = \{ \tau \}$, we distinguish two cases.
	\begin{itemize}
		\item Let $\tau = a$. We have that $d \in \{ a \}^{\Imc}$ iff $a$ denotes in $\Imc$ and $d = a^{\Imc}$. This means that $d \in \Delta^{\Imc}$ and $d = a^{\Imc}$. Equivalently, by definition of $\Imc'$, we have $d \in \De^{\Imc'}$ and $d = a^{\Imc'}$. The previous step means that $d \in (\De \sqcap \{ a^{\derel} \})^{\Imc'}$, i.e., $d \in (\{ a \}^{\derel})^{\Imc'}$.
		\item Let $\tau = \defdes D$. We have that $d \in \{ \defdes D \}^{\Imc}$ iff $\defdes D$ denotes in $\Imc$ and $d = (\defdes D)^{\Imc}$. Equivalently, $d \in \Delta^{\Imc}$ and $d = (\defdes D)^{\Imc}$, that is, $d \in \Delta^{\Imc}$ and $D^{\Imc} = \{ d \}$.
		In other words, we have $d \in \Delta^{\Imc}$, $d \in D^{\Imc}$, and, for all $e \in \Delta^{\Imc}$, $e \in D^{\Imc}$ implies $e = d$.
		By definition of $\Imc'$ and i.h., this means that $d \in (\De \sqcap D^{\derel})^{\Imc'}$ and, for all $e \in \Delta^{\Imc'}$, if $e \in (\De \sqcap D^{\derel})^{\Imc'}$, then $e = d$.
		This is equivalent to $(\De \sqcap D^{\derel})^{\Imc'} = \{ d \}$, meaning that
%		$d \in \De^{\Imc'}$,
		$\defdes (\De \sqcap D^{\derel})$ denotes in $\Imc'$ and $d = \defdes (\De \sqcap D^{\derel})^{\Imc'}$.
%		By definition of $\cdot^{\derel}$, the previous step is equivalent to:
%%		$d \in \De^{\Imc'}$,
%		$(\defdes D)^{\derel}$ denotes in $\Imc'$ and $d = ((\defdes D)^{\derel})^{\Imc'}$.
		Equivalently, we have
		$d \in(\{ \defdes (\De \sqcap D^{\derel}) \})^{\Imc'}$,
%		$d \in(\{ \defdes D^{\derel} \})^{\Imc'}$,
%		$d \in( \De \sqcap \{ \defdes D^{\derel} \})^{\Imc'}$,
		i.e., $d \in (\{ \defdes D \}^{\derel})^{\Imc'}$.
	\end{itemize}
%assume that $d \in \{ \tau
%  \}^{\Imc}$. Equivalently, $\tau$ denotes in $\Imc$ and
%  $d = \tau^{\Imc}$.  If $\tau$ is an individual name $a$, by
%  definition of $\Imc'$ we have that $a^{\Imc'} = a^{\Imc}$.  If
%  $\tau$ is a definite description $\defdes D$, by mutual induction on
%  $D$ one can show that, for any $e \in \Delta^{\Imc}$,
%  $e \in D^{\Imc}$ iff $e \in (D^{\exrel})^{\Imc'}$.  In both cases,
%  we obtain $(\tau^{\exrel})^{\Imc'} = \tau^{\Imc}$,\nb{A: holds just
%    on the restriction of $\Imc$ to $\Delta^{\Imc}$} and thus we have
%  that $d = \tau^{\Imc}$ is equivalent to
%  $d = (\tau^{\exrel})^{\Imc'}$. That is,
%  $d \in \{ \tau^{\exrel} \}^{\Imc'}$, which means
%  $d \in (\{ \tau \}^{\exrel})^{\Imc'}$.
\end{itemize}
%
%For the inductive case $C = \lnot D$, we have that, for $d \in \Delta^{\Imc}$, $d \in (\lnot D)^{\Imc}$ iff $d \not \in D^{\Imc}$.
%By i.h. and definition of $\Imc'$, the previous step means that
%%, for $d \in \De^{\Imc'}$,
%$d \not \in (D^{\derel})^{\Imc'}$, i.e.,
%%Equivalently,
%$d \in ((\lnot D)^{\derel})^{\Imc'}$.
%%$d \in \De^{\Imc'}$ and $d \in (\lnot D)^{\Imc'}$, i.e.,
%%$d \in (\De \sqcap \lnot D^{\derel})^{\Imc'}$, i.e., $d \in ((\lnot D)^{\derel})^{\Imc'}$.
%
The inductive cases $C = \lnot D$ and $C = D \sqcap E$ are straightforward. We show the remaining cases.
\begin{itemize}
	\item For $C = \exists r.D$, we have the following.
%
By definition,
%of $\exists r.D^{\Imc}$,
$d \in \exists r.D^{\Imc}$ iff $d \in \Delta^{\Imc}$ and there exists $e \in \Delta^{\Imc}$ such that $(d,e) \in r^{\Imc}$ and $e \in D^{\Imc}$. By i.h. and definition of $\Imc'$, this holds iff $d \in \De^{\Imc'}$ and there exists $e \in \De^{\Imc'}$ such that $(d,e) \in r^{\Imc'}$ and $e \in (D^{\derel})^{\Imc'}$, or, equivalently, iff $d \in \De^{\Imc'}$ and there exists $e \in \Delta^{\Imc'}$ such that $(d,e) \in r^{\Imc}$ and $e \in (\De \sqcap (D^{\derel}))^{\Imc'}$. This means that $d \in (\De \sqcap \exists r.(\De \sqcap D^{\derel}))^{\Imc'}$, which is the same as $d \in ((\exists r.D)^{\derel})^{\Imc'}$.
	\item The case of $C = \exists u.D$ is similar.
	\qedhere
\end{itemize}
%
\end{proof}




\begin{claim}
For every $C \sqsubseteq D \in \Omc$, $\Imc \models C \sqsubseteq D$ iff $\Imc' \models (C \sqsubseteq D)^{\derel}$.
\end{claim}
%
\begin{proof}
%The proof, by induction on $\psi$, is similar to the one given in Proposition~\ref{prop:dualdompartint}.
%\nb{M: todo fix/add}
%
%The proof is by induction on $\psi \in \sub{\p}$.
%
%For the base cases, without loss of generality, we can restrict ourselves to $\psi = C \sqsubseteq D$ only (cf. Section~\ref{sec:observations}).
%The base cases are as follows.
%We have the following.
%\nb{M: working here}
%
%\begin{itemize}
%	\item For $\psi = A(\tau)$, \ldots
%	\item For $\psi = r(\tau_{1}, \tau_{2})$, \ldots
We have that
%For $\psi = C \sqsubseteq D$,
$\Imc \models C \sqsubseteq D$ iff, for all $d \in \Delta^{\Imc}$, $d \in C^{\Imc}$ implies $d \in D^{\Imc}$. By definition of $\Imc'$ and the previous claim, this holds iff, for all $d \in \Delta^{\Imc'}$ such that $d \in \De^{\Imc'}$, $d \in (C^{\derel})^{\Imc'}$ implies $d \in (D^{\derel})^{\Imc'}$.
Equivalently, for all $d \in \Delta^{\Imc'}$, if $d \in (\De \sqcap C^{\derel})^{\Imc'}$, then $d \in (D^{\derel})^{\Imc'}$. The previous step means that $\Imc' \models \De \sqcap C^{\derel} \sqsubseteq D^{\derel}$, that is, $\Imc' \models (C \sqsubseteq D)^{\derel}$.
\qedhere
%\end{itemize}
%
%The inductive cases $\psi = \lnot \chi$ and $\psi = \chi \land \zeta$ are straightforward.
\end{proof}
%
Thanks to previous claim, from the assumption that $\Imc \models \Omc$ and the fact that $\Imc' \models \top \sqsubseteq \exists u.\De$, we can conclude that $\Imc' \models \Omc^{\derel}$.

%\nb{M: working here}

$(ii)$
%\nb{M: to fix, working here}
Let $\Jmc = (\Delta^{\Jmc}, \cdot^{\Jmc})$ be a total interpretation so that
$\Jmc \models \Omc^{\derel}$.
%$\Jmc \models \p^{-} \land  \lnot (\De \sqsubseteq \bot)$.
%
We define a partial interpretation $\Jmc' = (\Delta^{\Jmc'}, \cdot^{\Jmc'})$, where:
$\Delta^{\Jmc'} = \De^{\Jmc}$;
$A^{\Jmc'} = \De^{\Jmc} \cap A^{\Jmc}$, for every $A \in \NC$;
%\setminus \{ \De \}$
$r^{\Jmc'} = (\De^{\Jmc} \times \De^{\Jmc}) \cap r^{\Jmc} $, for every $r \in \NR$;
and, for every $a \in \NC$,
$a^{\Jmc'} = a^{\Jmc}$, if $a^{\Jmc} \in \De^{\Jmc}$, while 
%$a$ does not denote in $\Jmc'$,
$a^{\Jmc'}$
is undefined,
otherwise.
%
Observe that $\Delta^{\Jmc'}$ is well-defined, since $\Jmc \models \top \sqsubseteq \exists u.\De$.
%
We now claim the following.

\begin{claim}
For all $C \in \con{\Omc}$ and $d \in \Delta^{\Jmc}$, $d \in (C^{\derel})^{\Jmc}$ iff $d \in C^{\Jmc'}$. 
%For all $C \in \con{\p}$ and $d \in \Delta^{\Jmc'}$, $d \in C^{\Jmc'}$ iff $d \in (C^{\derel})^{\Jmc}$.
\end{claim}
%
\begin{proof}
The proof is by induction on $C$. The base cases are as follows.

\begin{itemize}
\item For $C = \bot$, $d \in (\bot^{\derel})^{\Jmc}$, i.e., $d \in \bot^{\Jmc}$, iff $d \in \bot^{\Jmc'}$.
\item For $C = \top$, we have that $d \in (\top^{\derel})^{\Jmc}$ iff, by definition of $\cdot^{\derel}$, $d \in (\De \sqcap \top)^{\Jmc}$. By definition of $\Jmc'$, this is equivalent to $d \in \top^{\Jmc'}$.
	\item For $C = A$, we have $d \in (A^{\derel})^{\Jmc}$ iff $d \in (\De \sqcap A)^{\Jmc}$, by definition of $\cdot^{\derel}$. This, by definition of $\Jmc'$, is equivalent to $d \in A^{\Jmc'}$.

	\item For $C = \{ \tau \}$, we distinguish two cases.
		\begin{itemize}
			\item Let $\tau = a$. We have that $d \in (\{ a \}^{\derel})^{\Jmc}$ iff, by definition of $\cdot^{\derel}$, $d \in (\De \sqcap \{ a \})^{\Jmc}$. Equivalently, $d \in \De^{\Jmc}$ and $d \in \{ a \}^{\Jmc}$, i.e., $d \in \De^{\Jmc}$ and $d = a^{\Jmc}$. By definition of $\Jmc'$, the previous step means that $a$ denotes in $\Jmc'$ and $d = a^{\Jmc'}$. That is, $d \in \{ a \}^{\Jmc'}$.
			
			\item Let $\tau = \defdes D$. We have that $d \in (\{ \defdes D \}^{\derel})^{\Jmc}$ iff, by definition of $\cdot^{\derel}$,
			$d \in \{ (\defdes D)^{\derel} \}^{\Jmc}$.
%			$d \in (\De \sqcap \{ \defdes D^{\derel} \})^{\Jmc}$.
			This means that
%			$d \in \De^{\Jmc}$,
			$(\defdes D)^{\derel}$ denotes in $\Jmc$ and $d = (\defdes D)^{\derel}$.
%			Again
			By definition of $\cdot^{\derel}$, the previous step is equivalent to
%			$d \in \De^{\Jmc}$ and
			$(\De \sqcap D^{\derel})^{\Jmc} = \{ d \}$. This means that
%			$d \in \De^{\Jmc}$,
			$d \in (\De \sqcap D^{\derel})^{\Jmc}$, and, for every $e \in \Delta^{\Jmc}$, $e \in (\De \sqcap D^{\derel})^{\Jmc}$ implies $e = d$.
			By i.h. and definition of $\Jmc'$, we have equivalently:
%			$d \in \Delta^{\Jmc'}$,
			$d \in (\Delta^{\Jmc'} \cap D^{\Jmc'})$, and, for every $e \in \Delta^{\Jmc}$, $e \in (\Delta^{\Jmc'} \cap D^{\Jmc'})$ implies $e = d$.
			The previous step can be equivalently rewritten as:
			$d \in \Delta^{\Jmc'}$, $d \in D^{\Jmc'}$, and, for every $e \in \Delta^{\Jmc'}$, $e \in D^{\Jmc'}$ implies $e = d$.
			This means that $D^{\Jmc'} = \{ d \}$, which in turn is equivalent to: $\defdes D$ denotes in $\Jmc'$ and $d = (\defdes D)^{\Jmc'}$.
			Equivalently, $d \in \{ \defdes D \}^{\Jmc'}$.
		\end{itemize}	
	
%	\item For $C = A$, let $d \in \Delta^{\Jmc'}$ and assume that $d \in A^{\Jmc'}$. Since, by definition,  $\Delta^{\Jmc'} = \De^{\Jmc}$ and $A^{\Jmc'} = \De^{\Jmc} \cap A^{\Jmc}$, the previous step is equivalent to $d \in A^{\Jmc}$ (if $d \in A^{\Jmc'}$, then clearly $d \in A^{\Jmc}$; and if $d \in A^{\Jmc}$, given that $d \in \Delta^{\Jmc'}$ and  $\Delta^{\Jmc'} = \De^{\Jmc}$, then $d \in A^{\Jmc'}$).
%This means that $d \in (A^{\derel})^{\Jmc}$.
%
%	\item For $C = \{ \tau \}$, consider $d \in \Delta^{\Jmc'}$ and assume that $d \in \{ \tau \}^{\Jmc'}$, i.e., $d = \tau^{\Jmc'}$. Given that $d \in \Delta^{\Jmc'}$ and $\Delta^{\Jmc'} = \De^{\Jmc}$, this means that $\tau^{\Jmc'} \in \De^{\Jmc}$.
%	If $\tau$ is an individual name $a$, we have by definition of $\Jmc'$ that $a^{\Jmc'} = a^{\Jmc}$.
%	If $\tau$ is a definite description $\defdes D$, by mutual induction it can be seen that $\defdes D^{\Jmc'} = (\defdes D^{\exrel})^{\Jmc}$.
%	In both cases, we have that $d = \tau^{\Jmc'}$ is equivalent to $d = (\tau^{\exrel})^{\Jmc}$. That is, $d \in \{ \tau^{\exrel} \}^{\Jmc}$, or, equivalently, $d \in (\{ \tau \}^{\exrel})^{\Jmc}$.
\end{itemize}

The inductive cases $C = \lnot D$, $C = D \sqcap E$ are straightforward. We show the remaining cases.

\begin{itemize}
	\item For $C = \exists r.D$, the following holds.
	We have that $d \in ((\exists r.D)^{\exrel})^{\Jmc}$ iff, by definition of $\cdot^{\derel}$, $d \in (\De \sqcap \exists r.(\De \sqcap D^{\derel}))^{\Jmc}$. This means that $d \in \De^{\Jmc}$ and there exists $e \in \Delta^{\Jmc}$ such that $(d,e) \in r^{\Jmc}$ and $e \in (\De \sqcap D^{\derel})^{\Jmc}$.
	Equivalently, $d \in \De^{\Jmc}$ and there exists $e \in \De^{\Jmc}$ such that $(d,e) \in r^{\Jmc}$ and $e \in (D^{\derel})^{\Jmc}$.
	By i.h. and definition of $\Jmc'$, since $\Delta^{\Jmc'} = \De^{\Jmc}$ and $r^{\Jmc'} = (\De^{\Jmc} \times \De^{\Jmc}) \cap r^{\Jmc}$, the previous step is equivalent to: $d \in \Delta^{\Jmc'}$ and there exists $e \in \Delta^{\Jmc'}$ such that $(d,e) \in r^{\Jmc'}$ and $e \in D^{\Jmc}$.
	This means that $d \in (\exists r.D)^{\Jmc'}$.
	\item The case of $C = \exists u.D$ is similar.
	\qedhere
%	\item For $C = \exists r.D$, the following holds.
%	We have that $d \in (\exists r.D)^{\Jmc'}$ iff there exists $e \in \Delta^{\Jmc'}$ such that $(d,e) \in r^{\Jmc'}$ and $e \in D^{\Jmc'}$.
%	By i.h. and definition of $\Jmc'$, since $\Delta^{\Jmc'} = \Ex^{\Jmc}$ and $r^{\Jmc'} = (\De^{\Jmc} \times \De^{\Jmc}) \cap r^{\Jmc}$, the previous step is equivalent to: there exists $e \in \Ex^{\Jmc}$ such that $(d,e) \in r^{\Jmc}$ and $e \in (D^{\exrel})^{\Jmc}$.
%	Equivalently, there exists $e \in \Delta^{\Jmc}$ such that $(d,e) \in r^{\Jmc}$ and $e \in (\Ex \sqcap D^{\exrel})^{\Jmc}$.
%	This means that $d \in (\exists r.(\Ex \sqcap D^{\exrel}))^{\Jmc}$, i.e., $d \in ((\exists r.D)^{\exrel})^{\Jmc}$.
\end{itemize}
\end{proof}

\begin{claim}
For every $C \sqsubseteq D \in \Omc$, $\Jmc' \models C \sqsubseteq D$ iff $\Jmc \models (C \sqsubseteq D)^{\derel}$.
\end{claim}
%
\begin{proof}
We have that $\Jmc' \models C \sqsubseteq D$ iff, for all $d \in \Delta^{\Jmc'}$, $d \in C^{\Jmc'}$ implies $d \in D^{\Jmc'}$. By definition of $\Jmc'$ and the previous claim, this holds iff, for all $d \in \Delta^{\Jmc}$ such that $d \in \De^{\Jmc}$, $d \in (C^{\derel})^{\Jmc}$ implies $d \in (D^{\derel})^{\Jmc}$.
Equivalently, for all $d \in \Delta^{\Jmc}$, if $d \in (\De \sqcap C^{\derel})^{\Jmc}$, then $d \in (D^{\derel})^{\Jmc}$. The previous step means that $\Jmc \models \De \sqcap C^{\derel} \sqsubseteq D^{\derel}$, that is, $\Jmc \models (C \sqsubseteq D)^{\derel}$.
%
\end{proof}

%As in the proof of $(i)$, using the previous claim, it can be seen by induction that $\Jmc' \models \psi$ iff $\Jmc \models \psi^{-}$, for every $\psi \in \sub{\p}$.
%%
%%{\color{red}{
%%Wrong! The previous claim indeed holds for $d \in \Delta^{\Jmc'}$, but this is not enough. Consider the instance query $[ A(a) ]$ and the total interpretation $\Jmc$ defined as follows (with every other concept, role and individual name arbitrarily interpreted):
%%\begin{itemize}
%%	\item $\Delta^{\Jmc} = \{ d, e \}$;
%%	\item $A^{\Jmc} = \{ d \}$;
%%	\item $\Ex^{\Jmc} = \{ e \}$;
%%	\item $a^{\Jmc} = d$.
%%\end{itemize}
%%We then construct the partial interpretation $\Jmc'$ by setting:
%%\begin{itemize}
%%	\item $\Delta^{\Jmc'} = \{ e \}$;
%%	\item $A^{\Jmc'} = \emptyset$;
%%	\item $a^{\Jmc'}$, undefined.
%%\end{itemize}
%%It holds that $\Jmc \models \{ a \} \sqsubseteq A$, i.e., $\Jmc \models [A(a)]^{+}$, but $\Jmc' \not \models [A(a)]$ (since $a$ does not denote in $\Jmc'$).
%%Therefore, Point $(ii)$ does not hold.
%%}
%%}
%%
Thanks to the claim above, since we have by assumption that $\Jmc \models \Omc^{\derel}$,
we can conclude that
$\Jmc' \models \Omc$.

\end{proof}

==> macros_old.tex <==
%%%
%%%
%%% SIDE COMMENTS ENVIRONMENT

\marginparwidth=15mm
\newcommand{\nb}[1]{\textcolor{red}{$|$}\mbox{}\marginpar
%{\scriptsize\raggedright\textcolor{red}{#1}}
{\parbox{18mm}{\scriptsize\textcolor{red}{\raggedright #1}}}
}


%%%
%%%
%%% PARAGRAPH ENVIRONMENT

\newcommand{\mypar}[1]{\medskip\noindent\textbf{#1.}}


%%%
%%%
%%% USEFUL SHORTCUTS / NOTATION

\newcommand{\e}{\emph}

\newcommand{\p}{\varphi}
\newcommand{\q}{\psi}
\newcommand{\s}{\sigma}

\newcommand{\eset}{\emptyset}
\newcommand{\mdl}{\models}
\newcommand{\Int}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\I}{\ensuremath{I}}

\newcommand{\sbs}{\subseteq}
\newcommand{\sqs}{\sqsubseteq}

\newcommand{\eqv}{\ensuremath{\doteq}\xspace}

\newcommand{\lp}{{\langle}}
\newcommand{\rp}{{\rangle}}

\newcommand{\tr}{^{\dagger}}
%\newcommand{\tr}{^{\ast}}
%\newcommand{\trx}{^{\dagger_{x}}}
%\newcommand{\try}{^{\dagger_{y}}}
\newcommand{\ttr}{^{\ddagger}}
\newcommand{\startr}{^{\star}}
\newcommand{\red}{^{\ast}}



\newcommand{\st}[2]{\ensuremath{{\pi}_{#1}(#2)}\xspace}



%%%
%%%
%%% VARIA


\newcommand{\concabbr}{\ensuremath{\bar{C}}\xspace}


\newcommand{\ass}[2]{\ensuremath{(#1 : #2)}\xspace}




\newcommand{\Isf}[1]{\ensuremath{\Imf^{#1}}\xspace}
%\newcommand{\Isf}[1]{\ensuremath{\Imf^{\mid^{#1}}}\xspace}

\newcommand{\Fsuf}[1]{\ensuremath{\Fmf^{#1}}\xspace}


%%%
%%%
%%% LOGIC


%%%
%%% SIGNATURE & SYNTACTIC NOTIONS

\newcommand{\sig}[1]{\ensuremath{\Sigma_{#1}}\xspace}

\newcommand{\size}[1]{\ensuremath{|#1|}\xspace}
\newcommand{\len}[1]{\ensuremath{{\sf len}(#1)}\xspace}

\newcommand{\sub}[1]{\ensuremath{\mathsf{for}(#1)}\xspace}
\newcommand{\subneg}[1]{\ensuremath{\mathsf{sub}_{\lnot}(#1)}\xspace}

\newcommand{\Var}{\ensuremath{\textsf{Var}}\xspace}

\newcommand{\ind}[1]{\ensuremath{\mathsf{ind}(#1)}\xspace}

\newcommand{\con}[1]{\ensuremath{\mathsf{con}(#1)}\xspace}
\newcommand{\conneg}[1]{\ensuremath{\mathsf{con}_{\lnot}(#1)}\xspace}
%\newcommand{\subc}[1]{\ensuremath{\mathsf{subc}(#1)}\xspace}

\newcommand{\ordcon}[1]{\ensuremath{\Cmf(#1)}\xspace}

\newcommand{\rol}[1]{\ensuremath{\mathsf{rol}(#1)}\xspace}

\newcommand{\atcon}[1]{\ensuremath{\mathsf{atcon}(#1)}\xspace}

\newcommand{\cons}[1]{\ensuremath{\mathsf{cons}(#1)}\xspace}


%%% SEMANTIC NOTIONS

\newcommand{\conseq}[1]{\ensuremath{\mathit{Cons}(#1)}\xspace}

\newcommand{\reduct}{\ensuremath{\Imf_{\mid_{\Sigma}}}\xspace}

\newcommand{\assign}{\ensuremath{\sigma}\xspace}
%\newcommand{\assign}{\ensuremath{\mathfrak{a}}\xspace}

\newcommand{\tvalue}{\ensuremath{\bar{\assign}}\xspace}

\newcommand{\dom}{\ensuremath{{\sf dom}}\xspace}



%%% TREES

\newcommand{\tree}[1]{\ensuremath{T_{#1}}\xspace}
\newcommand{\tvertex}{\ensuremath{V}\xspace}
\newcommand{\tedge}{\ensuremath{E}\xspace}
\newcommand{\tlabel}{\ensuremath{l}\xspace}
\newcommand{\leaf}[1]{\ensuremath{L(#1)}\xspace}
\newcommand{\fleaf}[1]{\ensuremath{f(#1)}\xspace}
\newcommand{\nleaf}[1]{\ensuremath{{\sf nl}(#1)}\xspace}
\newcommand{\vleaf}{\ensuremath{V}\xspace}


%%%
%%% LOGICAL OPERATORS


%\renewcommand{\U}{\ensuremath{\mathbin{\mathcal{U}}}\xspace}
\newcommand{\U}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\Until}{\ensuremath{\mathbin{\mathcal{U}}}\xspace}
\newcommand{\Since}{\ensuremath{\mathbin{\mathcal{S}}}\xspace}
\newcommand{\Wuntil}{\ensuremath{\mathbin{\mathcal{W}}}\xspace}

%\newcommand{\Next}{\ensuremath{\ocircle}}
\newcommand{\Next}{{\ensuremath{\raisebox{0.25ex}{\text{\scriptsize{$\bigcirc$}}}}}}
\newcommand{\nxt}{{\ensuremath{\raisebox{0.25ex}{\text{\scriptsize{$\bigcirc$}}}}}}
\newcommand{\Of}{\ocircle_{F}}
\newcommand{\Op}{\ocircle_{P}}
\newcommand{\Wnext}{\CIRCLE}

\newcommand{\D}{\Diamond}
\newcommand{\Df}{\D_{F}}
\newcommand{\Dp}{\Diamond_{P}}
\newcommand{\Dplus}{\ensuremath{\Diamond^{+}}\xspace}
\newcommand{\Uplus}{\ensuremath{\U^{+}}\xspace}
\newcommand{\B}{\Box}
\newcommand{\Bf}{\B_{F}}
\newcommand{\Bp}{\Box_{P}}

\newcommand{\Bast}{\boxast}

\newcommand{\monodic}{\ensuremath{\mathop{\ooalign{$\Box$ \cr \kern0.57ex \raisebox{0.2ex}{\scalebox{0.55}{$1$}}}\rule{0pt}{1.5ex} \kern-0.7ex}}\xspace}
%\newcommand{\monodic}{\ensuremath{(\textsf{m})}\xspace}


%%%
%%% LOGIC SYSTEMS AND LANGUAGES

\newcommand{\Lang}{\ensuremath{\mathcal{L}}}

%%% FIRST-ORDER LOGIC

\newcommand{\QL}{\ensuremath{\smash{\mathcal{QL}}}\xspace}
\newcommand{\QLd}{\ensuremath{\smash{\mathcal{QL}^{\defdes}_{\lambda}}}\xspace}

\newcommand{\fv}{\ensuremath{{\sf fv}}\xspace}


%%%
%%% DESCRIPTION LOGICS


\newcommand{\eq}[1]{\ensuremath{[{#1}]}\xspace} 
\newcommand{\indset}{\ensuremath{S}\xspace} 
\newcommand{\setind}{\ensuremath{\Gamma}\xspace}
\newcommand{\ra}{\ensuremath{{\cal R }_{\sf A}}}

\newcommand{\rolesucc}[2]{\ensuremath{#1^{#2}}\xspace} 


%%%
%%% SIGNATURE & SYNTACTIC NOTIONS

\newcommand{\NC}{\ensuremath{{\sf N_C}}\xspace}
\newcommand{\NI}{\ensuremath{{\sf N_I}}\xspace}
\newcommand{\NID}{\ensuremath{{\sf N_{I_{d}}}(\I)}\xspace}
\newcommand{\NR}{\ensuremath{{\sf N_R}}\xspace}
\newcommand{\NPr}{\ensuremath{\sf{N}_{\sf{P}}\xspace}}

\newcommand{\Roles}{\ensuremath{{\sf R}}\xspace}

\newcommand{\NIr}{\ensuremath{\textsf{N}_{\textsf{IR}}\xspace}}
\newcommand{\NIf}{\ensuremath{\textsf{N}_{\textsf{IF}}\xspace}}

%\newcommand{\funct}[1]{\ensuremath{(\mathsf{funct} \ #1)}\xspace}
\newcommand{\funct}[1]{\ensuremath{\top \sqsubseteq \ \leq \! 1 #1}\xspace}



%%% DESCRIPTION LOGICS LANGUAGES

\newcommand{\DLs}{\ensuremath{\textsf{DL}^{\defdes}}\xspace}

%\newcommand{\DL}{\ensuremath{\bf{DL}}\xspace}
\newcommand{\DL}{\ensuremath{\textsf{ExprDL}^{\defdes}}\xspace}
%\newcommand{\DL}{\ensuremath{\textsf{DL}^{\defdes}}\xspace}
%\newcommand{\DL}{\ensuremath{\textsf{DL}}\xspace}
%\newcommand{\DL}{\ensuremath{\text{DL}}\xspace}


\newcommand{\DLite}{\textsl{DL-Lite}\xspace}

\newcommand{\ExprDL}{\ensuremath{\textsf{ExpDL}^{\defdes}}\xspace}
\newcommand{\LightDL}{\ensuremath{\textsf{LightDL}^{\defdes}}\xspace}
%\newcommand{\ExprDL}{\ensuremath{\textsf{ExprDL}}\xspace}
%\newcommand{\LightDL}{\ensuremath{\textsf{LightDL}}\xspace}


\newcommand{\DLitea}{\ensuremath{\DLite_{\alpha}}}
\newcommand{\DLiteb}{\ensuremath{\DLite_\textit{bool}}}
\newcommand{\DLitek}{\ensuremath{\DLite_\textit{krom}}}
\newcommand{\DLitec}{\ensuremath{\DLite_\textit{core}}}


\newcommand{\ALC}{\ensuremath{\smash{\mathcal{ALC}}}\xspace}
\newcommand{\ALCO}{\ensuremath{\smash{\mathcal{ALCO}}}\xspace}
\newcommand{\ALCQI}{\ensuremath{\mathcal{ALCQI}}}
\newcommand{\DLR}{\ensuremath{\mathcal{DLR}}}
\newcommand{\ALCIO}{\ensuremath{\mathcal{ALCIO}}}
\newcommand{\ALCQO}{\ensuremath{\mathcal{ALCQO}}}
\newcommand{\ALCIQO}{\ensuremath{\mathcal{ALCIQO}}}

\newcommand{\ALCOu}{\ensuremath{\smash{\mathcal{ALCO}_{\!u}}}\xspace}
\newcommand{\ALCIOu}{\ensuremath{\mathcal{ALCIO}_{\!u}}}
\newcommand{\ALCQOu}{\ensuremath{\mathcal{ALCQO}_{\!u}}}

\newcommand{\ALCOud}{\ensuremath{\smash{\mathcal{ALCO}_{\!u}^{\defdes}}}\xspace}
\newcommand{\ALCIOud}{\ensuremath{\smash{\mathcal{ALCIO}_{\!u}^{\defdes}}}\xspace}


\newcommand{\ALCd}{\ensuremath{\smash{\mathcal{ALC}^{\defdes}}}\xspace}
\newcommand{\ALCOd}{\ensuremath{\smash{\mathcal{ALCO}^{\defdes}}}\xspace}
\newcommand{\ALCOdF}{\ensuremath{\smash{\mathcal{ALCO}^{\defdes}_{\Fmc}}}\xspace}
\newcommand{\ALCIOd}{\ensuremath{\smash{\mathcal{ALCIO}^{\defdes}}}\xspace}
\newcommand{\ALCQOd}{\ensuremath{\smash{\mathcal{ALCQO}^{\defdes}}}\xspace}
\newcommand{\ALCFOd}{\ensuremath{\smash{\mathcal{ALCFO}^{\defdes}_{\Fmc}}}\xspace}
\newcommand{\ALCIFOd}{\ensuremath{\smash{\mathcal{ALCIFO}^{\defdes}}}\xspace}
\newcommand{\ALCIQOd}{\ensuremath{\smash{\mathcal{ALCIQO}^{\defdes}}}\xspace}

\newcommand{\ALCOat}{\ensuremath{\smash{\mathcal{ALCO}@}}\xspace}


\newcommand{\EL}{\ensuremath{\smash{\mathcal{EL}}}\xspace}
\newcommand{\ELO}{\ensuremath{\smash{\mathcal{ELO}}}\xspace}
\newcommand{\ELOu}{\ensuremath{\smash{\mathcal{ELO}_{\!u}}}\xspace}

\newcommand{\ELOd}{\ensuremath{\smash{\mathcal{ELO}^{\defdes}}}\xspace}
\newcommand{\ELOud}{\ensuremath{\smash{\mathcal{ELO}_{u}^{\defdes}}}\xspace}
\newcommand{\ELOF}{\ensuremath{\smash{\mathcal{ELO}_{\Fmc}}}\xspace}
\newcommand{\ELOFd}{\ensuremath{\smash{\mathcal{ELOF}^{\defdes}}}\xspace}

\newcommand{\ELext}[3]{\ensuremath{\smash{\mathcal{EL{#1}}^{#2}_{\!#3}}}\xspace}



%%% QUASI-MODELS & REDUCTS

\newcommand{\nnf}{\ensuremath{\mathsf{nnf}}\xspace}
\newcommand{\cl}{\ensuremath{\mathsf{cl}}\xspace}

\newcommand{\clu}{\ensuremath{\cl^{\mathsf{u}}}\xspace}
\newcommand{\clc}{\ensuremath{\cl^{\mathsf{c}}}\xspace}
\newcommand{\clf}{\ensuremath{\cl^{\mathsf{f}}}\xspace}
\newcommand{\cls}{\ensuremath{\cl^\ast}\xspace}
\newcommand{\csub}{\ensuremath{\mathsf{csub}}\xspace}
\newcommand{\fsub}{\ensuremath{\mathsf{fsub}}\xspace}
\newcommand{\const}{\ensuremath{\ell_{\varphi}}\xspace}
\newcommand{\runSegments}[1]{\ensuremath{\mathsf{rs}(#1)}\xspace}
\newcommand{\roleConstraints}[1]{\ensuremath{\mathsf{rc}(#1)}\xspace}
\newcommand{\individuals}[1]{\NI(#1)}
\newcommand{\types}[1]{\mathsf{tp}(#1)}
\newcommand{\typesc}[1]{\mathsf{tp^{c}}(#1)}
\newcommand{\typesf}[1]{\mathsf{tp^{f}}(#1)}
\newcommand{\typescF}[1]{\mathsf{tp^{c}_{\Fmf}}(#1)}
\newcommand{\typesfF}[1]{\mathsf{tp^{f}_{\Fmf}}(#1)}
\newcommand{\quasistates}[1]{\mathsf{qs}(#1)}
\newcommand{\roles}[1]{\mathsf{rol}(#1)}
\newcommand{\rs}[1]{\ensuremath{\Rmc_{#1}}\xspace}


\newcommand{\real}{\ensuremath{{\sf real}}\xspace}



\newcommand{\quasimod}{\ensuremath{\Qmf}\xspace}
\newcommand{\setqm}[1]{\ensuremath{\Qmf(#1)}\xspace}
\newcommand{\setintqm}[1]{\ensuremath{\Imf(#1)}\xspace}

\newcommand{\runs}{\ensuremath{\Rmf}\xspace}

\newcommand{\stcand}{\ensuremath{\Cmf}\xspace}
\newcommand{\seqcand}{\ensuremath{\mathbf{q}}\xspace}

\newcommand{\ptcand}{\ensuremath{\Pmf}\xspace}

\newcommand{\modcand}{\ensuremath{S}\xspace}

\newcommand{\tp}{\ensuremath{t}\xspace}
\newcommand{\setcontp}{\ensuremath{\boldsymbol{T}}\xspace}
\newcommand{\setindtp}{\ensuremath{T^{con}}\xspace}

\newcommand{\basesetcontp}{\ensuremath{T}\xspace}
\newcommand{\copysetcontp}{\ensuremath{\tilde{T}}\xspace}
%\newcommand{\undersetcontp}{\ensuremath{T}\xspace}
\newcommand{\mult}{\ensuremath{m}\xspace}


\newcommand{\contp}{\ensuremath{{\boldsymbol{c}}}\xspace}
\newcommand{\fortp}{\ensuremath{{\boldsymbol{f}}}\xspace}




%%% CANONICAL MODELS

\newcommand{\paths}{\ensuremath{{\sf path}}\xspace}
\newcommand{\tail}{\ensuremath{{\sf tail}}\xspace}
\newcommand{\tlc}{\ensuremath{{\sf tlc}}\xspace}

\newcommand{\canmod}{\ensuremath{\Imc_{C,\Tmc}}\xspace}

\newcommand{\fincanmod}{\ensuremath{\Imc_{{\mathsf A},\Tmc}}\xspace}
%\newcommand{\fincanmod}{\ensuremath{\Imc_{F,\Tmc}}\xspace}
%\newcommand{\fincanmod}{\ensuremath{\Imc^{f}_{C,\Tmc}}\xspace}
\newcommand{\fincanmodvar}{\ensuremath{\Imc_{{\mathsf A},\Tmc'}}\xspace}






%%%
%%% MODAL LOGICS


%%% FRAMES AND MODELS

\newcommand{\FrL}{\ensuremath{\smash{\mathsf{Fr}\mathbf{L}}}\xspace}

\newcommand{\Fr}{\ensuremath{\smash{\mathcal{F}}}\xspace}


%%% MODAL LANGUAGES

\newcommand{\ML}{\ensuremath{\smash{\mathcal{ML}}}\xspace}
\newcommand{\QML}{\ensuremath{\smash{\mathcal{QML}}}\xspace}

\newcommand{\QMLd}{\ensuremath{\smash{\mathcal{QML}^{\defdes}_{\lambda}}}\xspace}

\newcommand{\MLALC}{\ensuremath{\smash{\ML_{\mathcal{ALC}}}}\xspace}

\newcommand{\MLnALC}[1]{\ensuremath{\smash{\ML^{#1}_{\mathcal{ALC}}}}\xspace}

\newcommand{\MLALCd}{\ensuremath{\smash{\ML_{\mathcal{ALC}^{\defdes}}}}\xspace}
\newcommand{\MLALCOd}{\ensuremath{\smash{\ML_{\mathcal{ALCO}^{\defdes}}}}\xspace}

%%% MODAL SYSTEMS

\newcommand{\EALC}{\ensuremath{\smash{\mathbf{E}_{\mathcal{ALC}}}}\xspace}
\newcommand{\MALC}{\ensuremath{\smash{\mathbf{M}_{\mathcal{ALC}}}}\xspace}
\newcommand{\KALC}{\ensuremath{\smash{\mathbf{K}_{\mathcal{ALC}}}}\xspace}
\newcommand{\KtwoALC}{\ensuremath{\smash{\mathbf{K}^{2}_{\mathcal{ALC}}}}\xspace}
\newcommand{\KthreeALC}{\ensuremath{\smash{\mathbf{K}^{3}_{\mathcal{ALC}}}}\xspace}

\newcommand{\KnALC}[1]{\ensuremath{\smash{\mathbf{K}^{#1}_{\mathcal{ALC}}}}\xspace}

\newcommand{\SfiveALCQI}{\ensuremath{\textbf{S5}_{\mathcal{ALCQI}}}}



%%%
%%% TEMPORAL LOGICS

%\newcommand{\QLog}[1]{\ensuremath{\textnormal{\textsf{QLog}}_{\Until}(#1)}\xspace}
\newcommand{\QLog}{\ensuremath{\textnormal{\textsf{QLog}}^{f}_{\Until}}\xspace}


\newcommand{\LTL}{\ensuremath{\textsl{LTL}}\xspace}
\newcommand{\LTLf}{\ensuremath{\LTL}\xspace}
%\newcommand{\LTLf}{\ensuremath{\LTL^{f}}\xspace}

\newcommand{\RVLTL}{\ensuremath{\textsl{RV-LTL}}\xspace}

%\newcommand{\QTL}{\ensuremath{\mathcal{QT\!L}}\xspace}
\newcommand{\QTL}{\ensuremath{{\textsl{T}_{\Until}\mathcal{QL}}}\xspace}


\newcommand{\QTLfr}[3]{\ensuremath{{\textsl{T}_{\Until}\mathcal{QL}^{#2}_{#3}}}\xspace}
%\newcommand{\QTLfr}[3]{\ensuremath{{\textsl{T}_{\Until}^{\ #1}\mathcal{QL}^{#2}_{#3}}}\xspace}
%\newcommand{\QTLfr}[3]{\ensuremath{\mathcal{\QTL}^{#1}_{#2}{#3}}\xspace}

\newcommand{\QTLn}[1]{\ensuremath{\smash{\QTL_{#1}}}\xspace}
%\newcommand{\QTLi}{{\ensuremath{\QTL^{1}}}}
%\newcommand{\QTLii}{{\ensuremath{\QTL^{2}}}}
%\newcommand{\QTLn}{{\ensuremath{\QTL^{n}}}}

\newcommand{\QTLm}{{\ensuremath{\QTL(\textsf{m})}}}
%\newcommand{\QTLiim}{{\ensuremath{\QTL^{2}(\textsf{m})}}}

\newcommand{\QTLf}{{\ensuremath{\QTL}}}
\newcommand{\QTLfn}[1]{\ensuremath{\smash{\QTL_{#1}}}\xspace}
%\newcommand{\QTLf}{{\ensuremath{\QTL^{f}}}}
%\newcommand{\QTLfn}[1]{\ensuremath{\smash{\QTL^{f}_{#1}}}\xspace}
%\newcommand{\QTLfi}{{\ensuremath{\QTL_{f}^{1}}}}
%\newcommand{\QTLfii}{{\ensuremath{\QTL_{f}^{2}}}}
%\newcommand{\QTLfn}{{\ensuremath{\QTL_{f}^{n}}}}

\newcommand{\QTLfm}{{\ensuremath{\QTLf(\textsf{m})}}}
\newcommand{\QTLfnm}{{\ensuremath{\QTLfn(\textsf{m})}}}
%\newcommand{\QTLfiim}{{\ensuremath{\QTL_{f}^{2}(\textsf{m})}}}

\newcommand{\QTLk}{{\ensuremath{\QTL^{k}}}}
\newcommand{\QTLkn}[1]{\ensuremath{\smash{\QTL^{k}_{#1}}}\xspace}



\newcommand{\TDL}{\ensuremath{\text{TDL}}\xspace}
\newcommand{\TDLs}{\ensuremath{\text{TDLs}}\xspace}
\newcommand{\TDLite}{\ensuremath{\textit{TDL-Lite}}\xspace}
\newcommand{\TDLitef}{\ensuremath{\textsl{TDL-Lite}_{\textit{f}}}\xspace}


\newcommand{\TuDLite}[2]{\ensuremath{\textsl{T}_{\Until}\DLite^{#1}_{#2}}\xspace}
\newcommand{\TfDLite}[1]{\ensuremath{\textsl{T}^{f}_{\Until}\DLite_{#1}}\xspace}
\newcommand{\TkDLite}[1]{\ensuremath{\textsl{T}^{k}_{\Until}\DLite_{#1}}\xspace}

%\newcommand{\TDLiteb}{\ensuremath{T_{\Until}\DLite_{bool}}\xspace}
%\newcommand{\TfDLiteb}{\ensuremath{T^{f}_{\Until}\DLite_{bool}}\xspace}
%\newcommand{\TkDLiteb}{\ensuremath{T^{k}_{\Until}\DLite_{bool}}\xspace}

\newcommand{\TusDLf}{\textsl{T}_{\mathcal{US}}\textit{DL}_{\textit{f}}}

\newcommand{\TALC}{\ensuremath{\smash{\textsl{T}_{\U}{\mathcal{ALC}}}}\xspace}
\newcommand{\TALCQI}{\ensuremath{\smash{\textsl{T}_{\U}{\mathcal{ALCQI}}}}}

\newcommand{\TALCf}{\ensuremath{\smash{\textsl{T}_{\U}{\mathcal{ALC}}}}\xspace}

\newcommand{\TALCk}{\ensuremath{\smash{\textsl{T}_{\U}{\mathcal{ALC}}}}\xspace}
\newcommand{\TALCfk}{\ensuremath{\smash{\textsl{T}_{\U}{\mathcal{ALC}}}}\xspace}

\newcommand{\TALCfg}{\ensuremath{\smash{\textsl{T}_{\U}(\textsf{g}){\mathcal{ALC}}}}\xspace}
\newcommand{\TALCfkg}{\ensuremath{\smash{\textsl{T}_{\U}(\textsf{g}){\mathcal{ALC}}}}\xspace}
%\newcommand{\TALCf}{\ensuremath{\smash{\textsl{T}^{f}_{\U}{\mathcal{ALC}}}}\xspace}
%
%\newcommand{\TALCk}{\ensuremath{\smash{\textsl{T}^{k}_{\U}{\mathcal{ALC}}}}\xspace}
%\newcommand{\TALCfk}{\ensuremath{\smash{\textsl{T}^{k}_{\U}{\mathcal{ALC}}}}\xspace}
%
%\newcommand{\TALCfg}{\ensuremath{\smash{\textsl{T}^{f}_{\U}(\textsf{g}){\mathcal{ALC}}}}\xspace}
%\newcommand{\TALCfkg}{\ensuremath{\smash{\textsl{T}^{k}_{\U}(\textsf{g}){\mathcal{ALC}}}}\xspace}

\newcommand{\TALCfB}{\ensuremath{\smash{\textsl{T}^{f}_{\Box}{\mathcal{ALC}}}}\xspace}

\newcommand{\TuALC}[1]{\ensuremath{\smash{\textsl{T}^{#1}_{\U}{\mathcal{ALC}}}}\xspace}



%%%
%%% MONODIC AXIOMS

\newcommand{\monod}{\ensuremath{\smash{\textnormal{\textit{\textbf{T}}}_{\U}{\textnormal{\textbf{QL}}_{\monodic}}}}\xspace}


%%%
%%% FINITE VS INFINITE TRACES

\newcommand{\finit}[2]{\textnormal{\ensuremath{\smash{\textsf{F}_{#1 #2}}}\xspace}}
\newcommand{\infinit}[2]{\textnormal{\ensuremath{\smash{\textsf{I}_{#1 #2}}}\xspace}}

\newcommand{\last}{\ensuremath{\textit{last}}\xspace}

\newcommand{\Pre}{\ensuremath{\textit{Pre}}\xspace}
\newcommand{\Prel}[1]{\ensuremath{\Pre_{l \geq #1}}\xspace}

\newcommand{\Ext}{\ensuremath{\textit{Ext}}\xspace}

\newcommand{\satfin}[1]{\ensuremath{\textsc{sat}_{f}(#1)}\xspace}
\newcommand{\satinf}[1]{\ensuremath{\textsc{sat}_{i}(#1)}\xspace}

\newcommand{\equivfin}[2]{\ensuremath{#1 \equiv_{\Fmf} #2}\xspace}
\newcommand{\equivinf}[2]{\ensuremath{#1  \equiv_{\Imf} #2}\xspace}
%\newcommand{\equivfin}[2]{\ensuremath{\textsc{equ}_{f}(#1, #2)}\xspace}
%\newcommand{\equivinf}[2]{\ensuremath{\textsc{equ}_{i}(#1, #2)}\xspace}


%%%
%%% DEFINITE DESCRIPTIONS

\newcommand{\NIInt}{\ensuremath{{\sf N}_{\sf I}^{\Imc}}\xspace}

\newcommand{\Ex}{\ensuremath{\mathsf{Ex}}\xspace}

\newcommand{\De}{\ensuremath{\mathsf{De}}\xspace}
%\newcommand{\De}{\ensuremath{\mathsf{Ex}}\xspace}


\newcommand{\exrel}{\ensuremath{\downarrow\Ex}\xspace}

\newcommand{\derel}{\ensuremath{\downarrow\De}\xspace}


\newcommand{\OutDom}{\ensuremath{\Delta}\xspace}
\newcommand{\InnDom}{\ensuremath{\mathfrak{d}}\xspace}

%\newcommand{\defdes}{\ensuremath{\smash{\textit{\riota \,}}}\xspace}
\newcommand{\defdes}{\ensuremath{\smash{\iota}}\xspace}

\newcommand{\concgzero}{\ensuremath{C^{\geq 1}_{\tau}}\xspace}
\newcommand{\concleqone}{\ensuremath{C^{\leq 1}_{\tau}}\xspace}
\newcommand{\conceqone}{\ensuremath{C^{= 1}_{\tau}}\xspace}


\newcommand{\topex}{\boldsymbol{{\mathsf{T}}}}
%\newcommand{\topex}{{\rotatebox[origin=c]{-90}{$\models$}}}

\newcommand{\simul}{\ensuremath{\leq}}



%%%
%%% PARTIAL CLOSED WORLD ASSUMPTION

\newcommand{\pcwmodels}{\mathbin{\ensuremath{\smash{\models_{{\sf PCWA}(\Sigma)}}}}\xspace}

%%%
%%%
%%% COMPLEXITY

\newcommand{\ACz}{{\ensuremath{\textsc{AC}^0}}}
\newcommand{\LogSpace}{\textsc{LogSpace}}
\newcommand{\NLogSpace}{\textsc{NLogSpace}}
\newcommand{\PTime}{\textsc{PTime}}
\newcommand{\NP}{\textsc{NP}}
\newcommand{\PSpace}{\textsc{PSpace}}
\newcommand{\ExpTime}{\textsc{ExpTime}}
\newcommand{\TwoExpTime}{\ensuremath{2\textsc{ExpTime}}}
\newcommand{\NExpTime}{\textsc{NExpTime}}
\newcommand{\ExpSpace}{\textsc{ExpSpace}}
\newcommand{\expsp}{\textsc{ExpSpace}}


%%%
%%%
%%% SANS-SERIF LETTERS

\newcommand{\Asf}{\ensuremath{\textsf{A}}\xspace}
\newcommand{\Bsf}{\ensuremath{\textsf{B}}\xspace}
\newcommand{\Csf}{\ensuremath{\textsf{C}}\xspace}
\newcommand{\Dsf}{\ensuremath{\textsf{D}}\xspace}
\newcommand{\Esf}{\ensuremath{\textsf{E}}\xspace}
\newcommand{\Fsf}{\ensuremath{\textsf{F}}\xspace}


%%%
%%%
%%% FRAKTUR LETTERS

\newcommand{\Amf}{\ensuremath{\mathfrak{A}}\xspace}
\newcommand{\Bmf}{\ensuremath{\mathfrak{B}}\xspace}
\newcommand{\Cmf}{\ensuremath{\mathfrak{C}}\xspace}
\newcommand{\Dmf}{\ensuremath{\mathfrak{D}}\xspace}
\newcommand{\Emf}{\ensuremath{\mathfrak{E}}\xspace}
\newcommand{\Fmf}{\ensuremath{\mathfrak{F}}\xspace}
\newcommand{\Gmf}{\ensuremath{\mathfrak{G}}\xspace}
\newcommand{\Hmf}{\ensuremath{\mathfrak{H}}\xspace}
\newcommand{\Imf}{\ensuremath{\mathfrak{I}}\xspace}
\newcommand{\Jmf}{\ensuremath{\mathfrak{J}}\xspace}
\newcommand{\Kmf}{\ensuremath{\mathfrak{K}}\xspace}
\newcommand{\Lmf}{\ensuremath{\mathfrak{L}}\xspace}
\newcommand{\Mmf}{\ensuremath{\mathfrak{M}}\xspace}
\newcommand{\Nmf}{\ensuremath{\mathfrak{N}}\xspace}
\newcommand{\Omf}{\ensuremath{\mathfrak{O}}\xspace}
\newcommand{\Pmf}{\ensuremath{\mathfrak{P}}\xspace}
\newcommand{\Qmf}{\ensuremath{\mathfrak{Q}}\xspace}
\newcommand{\Rmf}{\ensuremath{\mathfrak{R}}\xspace}
\newcommand{\Smf}{\ensuremath{\mathfrak{S}}\xspace}
\newcommand{\Tmf}{\ensuremath{\mathfrak{T}}\xspace}
\newcommand{\Umf}{\ensuremath{\mathfrak{U}}\xspace}
\newcommand{\Vmf}{\ensuremath{\mathfrak{V}}\xspace}
\newcommand{\Wmf}{\ensuremath{\mathfrak{W}}\xspace}
\newcommand{\Xmf}{\ensuremath{\mathfrak{X}}\xspace}
\newcommand{\Ymf}{\ensuremath{\mathfrak{Y}}\xspace}
\newcommand{\Zmf}{\ensuremath{\mathfrak{Z}}\xspace}

\newcommand{\FEmf}{\ensuremath{\Fmf \cdot_{E} \Emf}\xspace}
\newcommand{\FEmfC}{\ensuremath{\Fmf \cdot_{E} \Emf}\xspace}
\newcommand{\FImf}{\ensuremath{\Fmf \cdot \Imf}\xspace}
\newcommand{\FEImf}{\ensuremath{\Fmf \cdot_{E} \Imf}\xspace}



%%%
%%%
%%% MATHCAL LETTERS

\newcommand{\Amc}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\Bmc}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\Cmc}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\Dmc}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\Emc}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\Fmc}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\Gmc}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\Hmc}{\ensuremath{\mathcal{H}}\xspace}
\newcommand{\Imc}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\Jmc}{\ensuremath{\mathcal{J}}\xspace}
\newcommand{\Kmc}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\Lmc}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\Mmc}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\Nmc}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\Omc}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\Pmc}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\Qmc}{\ensuremath{\mathcal{Q}}\xspace}
\newcommand{\Rmc}{\ensuremath{\mathcal{R}}\xspace}
\newcommand{\Smc}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\Tmc}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\Umc}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\Vmc}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\Wmc}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\Xmc}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\Ymc}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\Zmc}{\ensuremath{\mathcal{Z}}\xspace}

\newcommand{\FEmc}{\ensuremath{\Fmc \cdot_{E} \Emc}}
\newcommand{\FImc}{\ensuremath{\Fmc \cdot \Imc}}
\newcommand{\FEImc}{\ensuremath{\Fmc \cdot_{E} \Imc}\xspace}


%%%
%%%
%%% BLACKBOARD LETTERS 

\newcommand{\Abl}{\ensuremath{\mathbb{A}}\xspace}
\newcommand{\Bbl}{\ensuremath{\mathbb{B}}\xspace}
\newcommand{\Cbl}{\ensuremath{\mathbb{C}}\xspace}
\newcommand{\Dbl}{\ensuremath{\mathbb{D}}\xspace}
\newcommand{\Ebl}{\ensuremath{\mathbb{E}}\xspace}
\newcommand{\Fbl}{\ensuremath{\mathbb{F}}\xspace}
\newcommand{\Gbl}{\ensuremath{\mathbb{G}}\xspace}
\newcommand{\Hbl}{\ensuremath{\mathbb{H}}\xspace}
\newcommand{\Ibl}{\ensuremath{\mathbb{I}}\xspace}
\newcommand{\Jbl}{\ensuremath{\mathbb{J}}\xspace}
\newcommand{\Kbl}{\ensuremath{\mathbb{K}}\xspace}
\newcommand{\Lbl}{\ensuremath{\mathbb{L}}\xspace}
\newcommand{\Mbl}{\ensuremath{\mathbb{M}}\xspace}
\newcommand{\Nbl}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\Obl}{\ensuremath{\mathbb{O}}\xspace}
\newcommand{\Pbl}{\ensuremath{\mathbb{P}}\xspace}
\newcommand{\Qbl}{\ensuremath{\mathbb{Q}}\xspace}
\newcommand{\Rbl}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\Sbl}{\ensuremath{\mathbb{S}}\xspace}
\newcommand{\Tbl}{\ensuremath{\mathbb{T}}\xspace}
\newcommand{\Ubl}{\ensuremath{\mathbb{U}}\xspace}
\newcommand{\Vbl}{\ensuremath{\mathbb{V}}\xspace}
\newcommand{\Wbl}{\ensuremath{\mathbb{W}}\xspace}
\newcommand{\Xbl}{\ensuremath{\mathbb{X}}\xspace}
\newcommand{\Ybl}{\ensuremath{\mathbb{Y}}\xspace}
\newcommand{\Zbl}{\ensuremath{\mathbb{Z}}\xspace}


%%%
%%%
%%% BOLDFACE LETTERS

\newcommand{\Abf}{\ensuremath{\mathbf{A}}\xspace}
\newcommand{\Bbf}{\ensuremath{\mathbf{B}}\xspace}
\newcommand{\Cbf}{\ensuremath{\mathbf{C}}\xspace}
\newcommand{\Dbf}{\ensuremath{\mathbf{D}}\xspace}
\newcommand{\Ebf}{\ensuremath{\mathbf{E}}\xspace}
\newcommand{\Fbf}{\ensuremath{\mathbf{F}}\xspace}
\newcommand{\Gbf}{\ensuremath{\mathbf{G}}\xspace}
\newcommand{\Hbf}{\ensuremath{\mathbf{H}}\xspace}
\newcommand{\Ibf}{\ensuremath{\mathbf{I}}\xspace}
\newcommand{\Jbf}{\ensuremath{\mathbf{J}}\xspace}
\newcommand{\Kbf}{\ensuremath{\mathbf{K}}\xspace}
\newcommand{\Lbf}{\ensuremath{\mathbf{L}}\xspace}
\newcommand{\Mbf}{\ensuremath{\mathbf{M}}\xspace}
\newcommand{\Nbf}{\ensuremath{\mathbf{N}}\xspace}
\newcommand{\Obf}{\ensuremath{\mathbf{O}}\xspace}
\newcommand{\Pbf}{\ensuremath{\mathbf{P}}\xspace}
\newcommand{\Qbf}{\ensuremath{\mathbf{Q}}\xspace}
\newcommand{\Rbf}{\ensuremath{\mathbf{R}}\xspace}
\newcommand{\Sbf}{\ensuremath{\mathbf{S}}\xspace}
\newcommand{\Tbf}{\ensuremath{\mathbf{T}}\xspace}
\newcommand{\Ubf}{\ensuremath{\mathbf{U}}\xspace}
\newcommand{\Vbf}{\ensuremath{\mathbf{V}}\xspace}
\newcommand{\Wbf}{\ensuremath{\mathbf{W}}\xspace}
\newcommand{\Xbf}{\ensuremath{\mathbf{X}}\xspace}
\newcommand{\Ybf}{\ensuremath{\mathbf{Y}}\xspace}
\newcommand{\Zbf}{\ensuremath{\mathbf{Z}}\xspace}

\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}} 
\newcommand{\Nbb}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\Zbb}{\ensuremath{\mathbb{Z}}\xspace}





%%%
%%%
%%% USELESS

\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\K}{\ensuremath{\mathcal{K}}}
\newcommand{\T}{\ensuremath{\mathcal{T}}}
\newcommand{\LL}{\ensuremath{\mathcal{L}}}

%
%\newcommand{\QT}{Q_\T}
%\newcommand{\QA}{Q_\A}
%
%\newcommand{\TuDLbn}{\ensuremath{\smash{\textsl{T}_{\mathcal{US}}\DLbn}}}%
%\newcommand{\TuDLcn}{\ensuremath{\smash{\textsl{T}_{\mathcal{US}}\DLcn}}}%
%
%\newcommand{\TdDLan}{\ensuremath{\smash{\textsl{T}_{F\!P}\DLan}}}%
%\newcommand{\TdDLbn}{\ensuremath{\smash{\textsl{T}_{F\!P}\DLbn}}}%
%\newcommand{\TdDLkn}{\ensuremath{\smash{\textsl{T}_{F\!P}\DLkn}}}%
%\newcommand{\TdDLcn}{\ensuremath{\smash{\textsl{T}_{F\!P}\DLcn}}}%
%
%\newcommand{\TdDLaHN}{\ensuremath{\smash{\textsl{T}_{\U\!\S}\rDLaHN}}}%
%\newcommand{\TdDLbHN}{\ensuremath{\smash{\textsl{T}_{\U\!\S}\rDLbHN}}}%
%\newcommand{\TdDLkHN}{\ensuremath{\smash{\textsl{T}_{\U\!\S}\rDLkHN}}}%
%\newcommand{\TdDLcHN}{\ensuremath{\smash{\textsl{T}_{\U\!\S}\rDLcHN}}}%
%
%\newcommand{\TdxDLan}{\ensuremath{\smash{\textsl{T}_{F\!P\!X}\DLan}}}
%\newcommand{\TdxDLbn}{\ensuremath{\smash{\textsl{T}_{F\!P\!X}\DLbn}}}%
%\newcommand{\TdxDLkn}{\ensuremath{\smash{\textsl{T}_{F\!P\!X}\DLkn}}}%
%\newcommand{\TdxDLcn}{\ensuremath{\smash{\textsl{T}_{F\!P\!X}\DLcn}}}%
%
%\newcommand{\zSVDLan}{\ensuremath{\smash{\textsl{T}_{U}\DLan}}}%
%\newcommand{\zSVDLb}{\ensuremath{\smash{\textsl{T}_{U}\DLbn}}}%
%\newcommand{\zSVDLk}{\ensuremath{\smash{\textsl{T}_{U}\DLkn}}}%
%\newcommand{\zSVDLc}{\ensuremath{\smash{\textsl{T}_{U}\DLcn}}}%
%
%\newcommand{\TxDLbn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{X}\DLbn}}}%
%\newcommand{\TdrDLbn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{F\!P}\DLbn}}}%
%\newcommand{\TurDLbn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{U}\DLbn}}}%
%
%\newcommand{\TdxrDLcn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{F\!P\!X}\DLcn}}}%
%\newcommand{\TdxrDLkn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{F\!P\!X}\DLkn}}}%


